\'Eclair -- Extracting Content and Layout with Integrated Reading Order for Documents

Optical Character Recognition (OCR) technology is widely used to extract text from images of documents, facilitating efficient digitization and data retrieval. However, merely extracting text is insufficient when dealing with complex documents. Fully comprehending such documents requires an understanding of their structure -- including formatting, formulas, tables, and the reading order of multiple blocks and columns across multiple pages -- as well as semantic information for detecting elements like footnotes and image captions. This comprehensive understanding is crucial for downstream tasks such as retrieval, document question answering, and data curation for training Large Language Models (LLMs) and Vision Language Models (VLMs). To address this, we introduce \'Eclair, a general-purpose text-extraction tool specifically designed to process a wide range of document types. Given an image, \'Eclair is able to extract formatted text in reading order, along with bounding boxes and their corresponding semantic classes. To thoroughly evaluate these novel capabilities, we introduce our diverse human-annotated benchmark for document-level OCR and semantic classification. \'Eclair achieves state-of-the-art accuracy on this benchmark, outperforming other methods across key metrics. Additionally, we evaluate \'Eclair on established benchmarks, demonstrating its versatility and strength across several evaluation standards.

==> sec/X_metrics_code.tex <==
\subsection{Reference code for confusion matrix metrics}

\begin{lstlisting}[
    caption=iou\_conf\_mat.py,
    basicstyle=\tiny,
    language=python,
    keepspaces=true,
    showspaces=false,
    showstringspaces=false
]
from typing import Optional

import torch
from scipy.optimize import linear_sum_assignment
from torchvision.ops.boxes import box_iou


def compute_iou_confusion_matrix(
        target_boxes: torch.Tensor,
        pred_boxes: torch.Tensor,
        target_classes: torch.Tensor,
        pred_classes: torch.Tensor,
        num_classes: int,
        iou_threshold: float = 0.5,
        confusion_matrix: Optional[torch.Tensor] = None,
) -> torch.Tensor:
    """
    Computes the confusion matrix for the given bounding boxes and classes.
    Will compute the IoU, and assign the best matching boxes to each other
    using Hungarian Matching.
    If the IoU is less than the threshold, the box will be considered as a
    false positive.

    Args:
        target_boxes: tensor of shape (num_targets, 4<x1, y1, x2, y2>)
        pred_boxes: tensor of shape (num_preds, 4<x1, y1, x2, y2>)
        target_classes: tensor of shape (num_targets,)
        pred_classes: tensor of shape (num_preds,)
        num_classes: number of classes
        iou_threshold: threshold for iou
        confusion_matrix: tensor of shape  (num_classes + 1, num_classes + 1),
            where +1 is the unmatched (background) class. The rows are 
            the target classes, and the columns are the predicted classes.
            If None, a new tensor will be created.
    
    Returns:
        confusion_matrix: tensor of shape (num_classes + 1, num_classes + 1),
            where +1 is the unmatched (background) class. The rows are 
            the target classes, and the columns are the predicted classes.
    """
    if confusion_matrix is None:
        confusion_matrix = torch.zeros(
            num_classes + 1, num_classes + 1, dtype=torch.int64
        )

    if (target_boxes.ndim == 0 or len(target_boxes) == 0) and \
            (pred_boxes.ndim == 0 or len(pred_boxes) == 0):
        return confusion_matrix
    elif pred_boxes.ndim == 0 or len(pred_boxes) == 0:
        for i in target_classes:
            confusion_matrix[i, -1] += 1
        return confusion_matrix
    elif target_boxes.ndim == 0 or len(target_boxes) == 0:
        for j in pred_classes:
            confusion_matrix[-1, j] += 1
        return confusion_matrix

    iou = box_iou(target_boxes, pred_boxes)
    iou[~(iou > 0)] = 0

    target_idx, pred_idx = linear_sum_assignment(-iou.cpu().numpy())
    # Find unassigned indexes
    # pred_idx is sorted!
    pred_idx = torch.tensor(pred_idx, dtype=torch.int64)
    target_idx = torch.tensor(target_idx, dtype=torch.int64)
    unassigned_pred = torch.ones(len(pred_classes), dtype=torch.bool)
    unassigned_pred[pred_idx] = False
    unassigned_target = torch.ones(len(target_classes), dtype=torch.bool)
    unassigned_target[target_idx] = False

    for i in range(len(target_classes)):
        if unassigned_target[i]:
            confusion_matrix[target_classes[i], -1] += 1
    for j in range(len(pred_classes)):
        if unassigned_pred[j]:
            confusion_matrix[-1, pred_classes[j]] += 1

    iou_mask = iou > iou_threshold
    for i, j in zip(target_idx, pred_idx):
        if iou_mask[i, j]:
            confusion_matrix[target_classes[i], pred_classes[j]] += 1
        else:
            confusion_matrix[target_classes[i], -1] += 1
            confusion_matrix[-1, pred_classes[j]] += 1

    return confusion_matrix
\end{lstlisting}

\begin{lstlisting}[
    caption=conf\_mat.py,
    basicstyle=\tiny,
    language=python,
    keepspaces=true,
    showspaces=false,
    showstringspaces=false
]
from typing import Optional, Sequence
import torch


class ConfusionMatrix:
    # NxN confusion matrix
    confusion_matrix: torch.Tensor

    # True positive for each class. The true positives represent the number of
    # predictions that were matched to a target.
    tp: torch.Tensor

    # False positive for each class. The false positives represent the number of
    # predictions that were not matched to a target.
    fp: torch.Tensor

    # False negative for each class. The false negatives represent the number of
    # targets that were not matched to a prediction.
    fn: torch.Tensor

    # True negative for each class. The true negatives represent the number of
    # predictions that were not matched to a target.
    tn: torch.Tensor

    # Total number of predictions for each class
    sum_preds: torch.Tensor

    # Total number of targets for each class
    sum_targets: torch.Tensor

    # The sum of the confusion matrix.
    samples: torch.Tensor

    # The sum of the true positives.
    correct: torch.Tensor

    # Precision for each class
    _class_precision: Optional[torch.Tensor] = None

    # Recall for each class
    _class_recall: Optional[torch.Tensor] = None

    def __init__(self, confusion_matrix: torch.Tensor, last_is_no_match: bool) -> None:
        """
        Args:
            confusion_matrix: tensor of shape (num_classes + 1, num_classes + 1),
                where +1 is the unmatched (background) class. The rows are the
                target classes, and the columns are the predicted classes.
            last_is_no_match: If true, expect the last column/row to be the no
                match class.
        """
        self.confusion_matrix = confusion_matrix
        self.samples = self.confusion_matrix.sum()
        self.sum_preds = self.confusion_matrix.sum(dim=0)
        self.sum_targets = self.confusion_matrix.sum(dim=1)
        self.tp = self.confusion_matrix.diag()
        if last_is_no_match:
            # The counts are over all, but only consider the positive classes
            self.sum_preds = self.sum_preds[:-1]
            self.sum_targets = self.sum_targets[:-1]
            self.tp = self.tp[:-1]
        self.fp = self.sum_preds - self.tp
        self.fn = self.sum_targets - self.tp
        self.tn = self.samples - self.sum_preds - self.sum_targets + self.tp
        self.correct = self.tp.sum()

    @property
    def precision(self) -> torch.Tensor:
        """
        Returns the precision for each class.
        """
        if self._class_precision is None:
            self._class_precision = self.tp / torch.clamp(self.tp + self.fp, min=1)
        return self._class_precision

    @property
    def recall(self) -> torch.Tensor:
        """
        Returns the recall for each class.
        """
        if self._class_recall is None:
            self._class_recall = self.tp / torch.clamp(self.tp + self.fn, min=1)
        return self._class_recall

    @property
    def f1(self) -> torch.Tensor:
        """
        Returns the F1 score for each class.
        """
        return 2 * self.precision * self.recall / (self.precision + self.recall)

    @property
    def accuracy(self) -> torch.Tensor:
        """
        Returns the accuracy for each class.
        """
        return (self.tp + self.tn) / (self.tp + self.tn + self.fp + self.fn)

    @property
    def macro_precision(self) -> torch.Tensor:
        """
        Returns the macro precision.
        """
        return self.precision.mean()

    @property
    def balanced_accuracy(self) -> torch.Tensor:
        """
        Returns the balanced accuracy. This equals the macro recall.
        "how likely will an individual of that class be classified correctly?"
        """
        return self.recall.mean()
    
    @property
    def macro_f1(self) -> torch.Tensor:
        """
        Returns the macro F1 score. 
        "high Macro-F1 values indicate that the algorithm has good performance
        on all the classes, whereas low Macro-F1 values refers to poorly
        predicted classes."
        """
        return (
            2 * self.macro_precision * self.balanced_accuracy / 
            (1/self.macro_precision + 1/self.balanced_accuracy)
        )

    @property
    def overall_accuracy(self) -> torch.Tensor:
        """
        Returns the overall accuracy. This equals the micro-F1, micro-precision,
        and micro-recall.
        """
        return self.correct / self.samples

\end{lstlisting}
